Actionable and Interpretable Fault Localization for Recurring Failures in Online Service Systems

Fault localization is challenging in an online service system due to its monitoring data's large volume and variety and complex dependencies across or within its components (e.g., services or databases). Furthermore, engineers require fault localization solutions to be actionable and interpretable, which existing research approaches cannot satisfy. Therefore, the common industry practice is that, for a specific online service system, its experienced engineers focus on localization for recurring failures based on the knowledge accumulated about the system and historical failures. Although the above common practice is actionable and interpretable, it is largely manual, thus slow and sometimes inaccurate. In this paper, we aim to automate this practice through machine learning. That is, we propose an actionable and interpretable fault localization approach, DejaVu, for recurring failures in online service systems. For a specific online service system, DejaVu takes historical failures and dependencies in the system as input and trains a localization model offline; for an incoming failure, the trained model online recommends where the failure occurs (i.e., the faulty components) and which kind of failure occurs (i.e., the indicative group of metrics) (thus actionable), which are further interpreted by both global and local interpretation methods (thus interpretable). Based on the evaluation on 601 failures from three production systems and one open-source benchmark, in less than one second, DejaVu can on average rank the ground truths at 1.66-th to 5.03-th among a long candidate list, outperforming baselines by at least 51.51%.

==> ccb_tickets_table.tex <==
\begingroup
\setlength{\tabcolsep}{1.5pt} %
\renewcommand{\arraystretch}{1} %
\begin{table}[htb]
\caption{Summary of \num{527} closed failures tickets at \textit{compA}. Categories with less than two failures are omitted.}
\centering
\footnotesize
\begin{tabularx}{\columnwidth}{lX}
\thickhline
    Category & Description
\\
\thickhline
\greycell{}\begin{tabular}[c]{@{}l@{}}3rd-party service\\ unavailable\end{tabular} & The third-party services responds slowly. Operators need to find the root-cause service and notify its operators. \\
Bad request                     & Requests contain various illegal parameters or have missing parameters.\\
Configuration                   & Incorrect or non-optimized configurations. \\
Code defect                     & Codes do not meet the design goal or have bugs. The root causes varies.\\
Bursting workload             & Bursting workload causes various services overloaded.\\
Change                          & These failures are caused by software or configuration changes.\\
\greycell{}\begin{tabular}[c]{@{}l@{}}Database\\ /slow-query\end{tabular}              & \greycell{}These failures are caused by non-optimized SQL queries and can be fixed by optimizing the SQL queries. \\
\greycell{}Middleware                      &  \greycell{}These failures are caused by broken middlewares and can be fixed by restarting them.  \\
\greycell{}Memory/usage                    & \greycell{}These failures are caused by insufficient free memory  space on some servers. \\
\greycell{}Disk                            & \greycell{}These failures are caused failing disks and can be mitigated by replacing them.\\
Jitter                          & Network jitter. Usually these failures recover without any operation from operators.\\
\greycell{}Network/cable                   & \greycell{}These failures are caused broken cables and can be mitigated by replacing them.\\
Inconsistent data              & Inconsistent data, e.g., delayed account reconciliation. \\
Compatibility                   & Incompatible components. \\
\greycell{}\begin{tabular}[c]{@{}l@{}}Database\\ /missing-index\end{tabular}          & \greycell{}These failures are caused by missing or outdated indices and can be fixed by building/rebuilding the indices. \\
\greycell{}\begin{tabular}[c]{@{}l@{}}3rd-party-service\\ \greycell{}/quota\end{tabular}       & \greycell{}Caused by quotas of 3rd-party services.\\
\greycell{}Memory/failure                  & \greycell{}These failures are caused failing memories and can be mitigated by replacing them.\\
Scheduled job                   & A scheduled job (e.g., database backup) harms the performance\\
\thickhline
\end{tabularx}
\label{tbl:failures-in-comp-a}    
\end{table}
\endgroup


==> makefile <==
TEX_FILES = $(shell find . -name '*.tex')
MAIN_TEX = cfl.tex
TARGET_PDF = cfl.pdf
CROP_FIGURE_OPERATIONS = $(shell find 'figures' -name '*.pdf' | sed -E 's/(.*)/\1.crop/g' | sed 's/ /\\ /g')

.SECONDARY:

.PHONY: crop phony_explicit build sync

build: $(TARGET_PDF);

crop: $(CROP_FIGURE_OPERATIONS);

clean:
	latexmk --output-directory=. -C

sync:
	(git add -u && git commit -m "$(date) local update") || echo nothing to commit
	git pull --no-edit
	git push


%.crop: % phony_explicit
	pdfcrop $< $<

.PHONY: build
cfl.pdf: crop $(TEX_FILES)
	bash -c 'latexmk -C; latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX)'

